Barack's Wife Hillary: Using Knowledge-Graphs for Fact-Aware Language Modeling

Modeling human language requires the ability to not only generate fluent text but also encode factual knowledge. However, traditional language models are only capable of remembering facts seen at training time, and often have difficulty recalling them. To address this, we introduce the knowledge graph language model (KGLM), a neural language model with mechanisms for selecting and copying facts from a knowledge graph that are relevant to the context. These mechanisms enable the model to render information it has never seen before, as well as generate out-of-vocabulary tokens. We also introduce the Linked WikiText-2 dataset, a corpus of annotated text aligned to the Wikidata knowledge graph whose contents (roughly) match the popular WikiText-2 benchmark. In experiments, we demonstrate that the KGLM achieves significantly better performance than a strong baseline language model. We additionally compare different language model's ability to complete sentences requiring factual knowledge, showing that the KGLM outperforms even very large language models in generating facts.

==> fig/model-UNUSED.tex <==
\begin{tikzpicture}[node distance=1cm]

\tikzstyle{vvector} = [rectangle,minimum width=0.35cm,minimum height=1cm,draw]
\tikzstyle{hvector} = [rectangle,minimum width=0mm,inner sep=0mm,minimum height=0.35cm,draw=white]
\tikzstyle{sq} = [rectangle,minimum width=0.35cm,minimum height=0.35cm,draw]

% Text
\node (text) at (-3.5,3.5) {\em Super Mario Land is $\ldots$ published by $\underline{\hspace{10mm}}$};

\node[below] at (text.south east) {\textcolor{gray}{$x_t$}};
%\node (ct) [above,vvector,fill=blue!25] at ([yshift=0.5cm]text.north east) {};
%\node[left] at (ct.west) {\textcolor{gray}{$c_t$}};


% Type
\node (new) at (1.5,2) {\textcolor{gray}{$t_t$}};
\node (newb) [sq,fill=black!20,below] at (new.south) {};
\node (relb) [sq,fill=black!70,below] at (newb.south) {};
\node (nomb) [sq,fill=black!10,below] at (relb.south) {};
%\draw[->,-Circle,blue!25] (ct) -- (nomb);

\node[left of=newb,xshift=-1mm] {new entity};
\node[left of=relb,xshift=-3.3mm] {related entity};
\node[left of=nomb,xshift=-4mm] {not a mention};

% Not a mention
%\node[rectangle, draw=black] (textlstm) at ([xshift=1.5cm]ct.east) {LSTM};
%\draw[->] (nomb-sum) -- (textlstm.north);
%\draw[->] (ct) -- (textlstm);
%\draw[->] (textlstm) -- ([xshift=5cm]textlstm.east);
\node (nomint) at (5,0) {};
\draw[-] (nomb) -- (nomint.east);
\draw[->] (nomint) -- ([xshift=9.1cm]nomint.east) node[pos=0.5,above]{\textcolor{gray}{$e_t=\emptyset$}};

% New Entity
\node (allent) at (2.5,6) {Whole KG};
\node (allent1v) [below,hvector,fill=purple!25] at ([yshift=-0mm]allent.south) {};
\node (allent1t) [left] at ([xshift=-0.5mm]allent1v.west) {\scriptsize AAA\_Inc.};
\node (allent1b) [right,sq,fill=black!5] at ([xshift=2mm]allent1v.east) {};
\node (allent2v) [below,hvector,fill=purple!25] at ([yshift=-0mm]allent1v.south) {};
\node (allent2t) [left] at ([xshift=-0.5mm]allent2v.west) {\scriptsize Aardvark};
\node (allent2b) [right,sq,fill=black!85] at ([xshift=2mm]allent2v.east) {};
\node (aellipses) [below] at ([yshift=-2mm]allent2v) {$\ldots$};
\node (allent3v) [below,hvector,fill=purple!25] at ([yshift=-0mm]aellipses.south) {};
\node (allent3t) [left] at ([xshift=-0.5mm]allent3v.west) {\scriptsize Zzyzx,\_CA};
\node (allent3b) [right,sq,fill=black!10] at ([xshift=2mm]allent3v.east) {};
\node[circle,draw,inner sep=0mm] (aoplus) at (5,5) {$+$};
\draw[->] (allent1b) -- (aoplus);
\draw[->] (allent2b) -- (aoplus);
\draw[->] (allent3b) -- (aoplus);
\draw[-Circle] (newb) -- (aoplus);
\draw[->] (aoplus) -- ([xshift=9cm]aoplus.east) node[pos=0.5,above]{\textcolor{gray}{$e_t$}};
%\draw[->,-Circle,blue!25] (ct) -- (allent3bb);

% Related Entity (parent)
\node (pent) at (5.5,3.5) {Local Entities};
\node (pent1v) [below,hvector,fill=purple!25] at ([yshift=-0mm]pent.south) {};
\node (pent1t) [left] at ([xshift=-0.5mm]pent1v.west) {\scriptsize 1989};
\node (pent1b) [right,sq,fill=black!15] at ([xshift=2mm]pent1v.east) {};
\node (pent2v) [below,hvector,fill=purple!25] at ([yshift=-0mm]pent1v.south) {};
\node (pent2t) [left] at ([xshift=-0.5mm]pent2v.west) {\scriptsize Super Mario Land};
\node (pent2b) [right,sq,fill=black!75] at ([xshift=2mm]pent2v.east) {};
\node (pellipses) [below] at ([yshift=-2mm]pent2v) {$\ldots$};
\node (pent3v) [below,hvector,fill=purple!25] at ([yshift=-0mm]pellipses.south) {};
\node (pent3t) [left] at ([xshift=-0.5mm]pent3v.west) {\scriptsize platform video game};
\node (pent3b) [right,sq,fill=black!10] at ([xshift=2mm]pent3v.east) {};
\node[circle,draw,inner sep=0mm] (poplus) at (7,1.25) {$+$};
\draw[->] (pent1b) -- (poplus);
\draw[->] (pent2b) -- (poplus);
\draw[->] (pent3b) -- (poplus);
\draw[->,-Circle] (relb) -- (poplus);

% Related Entity (tail)
\node (tent) at (10.5,3.5) {Local KG};
\node (tent1v) [below,hvector,fill=purple!25] at ([yshift=-0mm]tent.south) {};
\node (tent1t) [left] at ([xshift=-0.5mm]tent1v.west) {{\scriptsize $\langle$SML, publisher, Nintendo$\rangle$}};
\node (tent1b) [right,sq,fill=black!80] at ([xshift=2mm]tent1v.east) {};
\node (tent2v) [below,hvector,fill=purple!25] at ([yshift=-0mm]tent1v.south) {};
\node (tent2t) [left] at ([xshift=-0.5mm]tent2v.west) {\scriptsize $\langle$SML, platform, GameBoy$\rangle$};
\node (tent2b) [right,sq,fill=black!15] at ([xshift=2mm]tent2v.east) {};
\node (tellipses) [below] at ([yshift=-2mm]tent2v) {$\ldots$};
\node (tent3v) [below,hvector,fill=purple!25] at ([yshift=-0mm]tellipses.south) {};
\node (tent3t) [left] at ([xshift=-0.5mm]tent3v.west) {\scriptsize $\langle$1989, partOf, 1980s$\rangle$};
\node (tent3b) [right,sq,fill=black!5] at ([xshift=2mm]tent3v.east) {};
\node[circle,draw,inner sep=0mm] (toplus) at (12,1.25) {$+$};
\draw[->] (tent1b) -- (toplus);
\draw[->] (tent2b) -- (toplus);
\draw[->] (tent3b) -- (toplus);
%\draw[->] (newb) -- (poplus);
\draw[->,-Circle] (poplus) -- (toplus) node[pos=0.5,above]{\textcolor{gray}{$p_t$}};
\draw[->] (toplus) -- ([xshift=2cm]toplus.east)node[pos=0.5,above]{\textcolor{gray}{$e_t$}};


% Output
\draw[-,gray] (14.5,-0.5) -- (14.5,5.5);
\node[right] at (15,2.5) {\textcolor{gray}{$x_t=$``Nintendo''}};

%\path pic[gray] (inpute) at ([yshift=1cm]env) {mysymbol};
%\node[rectangle, rounded corners, minimum height=0.5cm, minimum width=9cm,text centered, draw=black] (inpute)  at ([yshift=-0.5cm,xshift=2.5cm]env) {};
%    \filldraw[fill opacity=0] ([xshift=-0.25cm]inpute.east) circle (0.2cm);
%    \filldraw[fill opacity=1.0] ([xshift=-0.75cm]inpute.east) circle (0.2cm);
%    \node[below] at ([xshift=3.75cm]inpute.south) {\scriptsize \textcolor{gray}{emotion3}};
%    \filldraw[fill opacity=0] ([xshift=-1.25cm]inpute.east) circle (0.2cm);
%    \draw[dotted] ([xshift=3cm]inpute.north) -- ([xshift=3cm]inpute.south);

%	\filldraw[fill opacity=0] ([xshift=-1.75cm]inpute.east) circle (0.2cm);
%	\filldraw[fill opacity=0] ([xshift=-2.25cm]inpute.east) circle (0.2cm);
%    \node[below] at ([xshift=2.25cm]inpute.south) {\scriptsize \textcolor{gray}{profession3}};
%    \filldraw[fill opacity=1] ([xshift=-2.75cm]inpute.east) circle (0.2cm);
%    \draw ([xshift=1.5cm]inpute.north) -- ([xshift=1.5cm]inpute.south);

%\node (utt) at (2.25,0) {Utterance, $u$};
%\node (inputu) [input] at ([yshift=-0.5cm,xshift=-0.5cm]utt) {};
%    \node[below] at (inputu.south) {\scriptsize \textcolor{gray}{word embedding}};


% Hidden Layers
%\node (hidden1) [hidden] at (0,1) {$h_1$};
%\draw[->] (inpute) -- (hidden1);
%\draw[->] (inputu) -- (hidden1);
%\node (hidden2) [hidden, above of=hidden1] {$h_2$};
%\draw[->] (hidden1) -- (hidden2);
%\node (hidden3) [hidden, above of=hidden2] {$h_3$};
%\draw[->] (hidden2) -- (hidden3);

% Output Layers
%\node[rectangle, rounded corners, minimum height=0.5cm, minimum width=1.5cm,text centered, draw=black, above of=hidden3] (output) {};
%	\filldraw[fill opacity=0.1] ([xshift=-0.25cm]output.east) circle (0.2cm);
%    \filldraw[fill opacity=0.6] ([xshift=-0.75cm]output.east) circle (0.2cm);
%    \filldraw[fill opacity=0.2] ([xshift=-1.25cm]output.east) circle (0.2cm);
%    \node[above] at (output.north) {\scriptsize \textcolor{gray}{probabilities}};
%\draw[->] (hidden3) -- (output);
%\node[above of=output] (outputl) {Interpretation, $i$};


\end{tikzpicture}

